GenFusion: Closing the Loop between Reconstruction and Generation via Videos

Recently, 3D reconstruction and generation have demonstrated impressive novel view synthesis results, achieving high fidelity and efficiency. However, a notable conditioning gap can be observed between these two fields, e.g., scalable 3D scene reconstruction often requires densely captured views, whereas 3D generation typically relies on a single or no input view, which significantly limits their applications. We found that the source of this phenomenon lies in the misalignment between 3D constraints and generative priors. To address this problem, we propose a reconstruction-driven video diffusion model that learns to condition video frames on artifact-prone RGB-D renderings. Moreover, we propose a cyclical fusion pipeline that iteratively adds restoration frames from the generative model to the training set, enabling progressive expansion and addressing the viewpoint saturation limitations seen in previous reconstruction and generation pipelines. Our evaluation, including view synthesis from sparse view and masked input, validates the effectiveness of our approach. More details at https://genfusion.sibowu.com.

==> sec/5_conclusion.tex <==
\section{Conclusion}
\vspace{-0.17cm}
% We presented Mip-Splatting, a modification to 3D Gaussian Splatting, which introduces two novel filters, namely a 3D smoothing filter and a 2D Mip filter, to achieve alias-free rendering at arbitrary scales. Our 3D smoothing filter effectively limits the maximal frequency of Gaussian primitives to match the sampling constraints imposed by the training images, while the 2D Mip filter approximates the box filter to simulate the physical imaging process. Our experimental results demonstrate that Mip-Splatting is competitive with state-of-the-art methods in terms of performance when training and testing at the same scale / sampling rate. Importantly, it significantly outperforms state-of-the-art methods in out-of-distribution scenarios, when testing at sampling rates different from training, resulting in better generalization to out-of-distribution camera poses and zoom factors.
\red{We introduced Mip-Splatting, a technique improving 3DGS with a 3D smoothing filter and a 2D Mip filter for alias-free rendering at any scale. Our 3D smoothing filter effectively limits the maximal frequency of Gaussian primitives to match the sampling constraints imposed by the training images, while the 2D Mip filter approximates the box filter to simulate the physical imaging process.
Mip-Splatting significantly outperforms state-of-the-art methods in out-of-distribution scenarios, when testing at sampling rates different from training, resulting in better generalization to out-of-distribution camera poses and zoom factors.}
